Pentagon at MEDIQA 2019: Multi-task Learning for Filtering and Re-ranking Answers using Language Inference and Question Entailment

Parallel deep learning architectures like fine-tuned BERT and MT-DNN, have quickly become the state of the art, bypassing previous deep and shallow learning methods by a large margin. More recently, pre-trained models from large related datasets have been able to perform well on many downstream tasks by just fine-tuning on domain-specific datasets . However, using powerful models on non-trivial tasks, such as ranking and large document classification, still remains a challenge due to input size limitations of parallel architecture and extremely small datasets (insufficient for fine-tuning). In this work, we introduce an end-to-end system, trained in a multi-task setting, to filter and re-rank answers in the medical domain. We use task-specific pre-trained models as deep feature extractors. Our model achieves the highest Spearman's Rho and Mean Reciprocal Rank of 0.338 and 0.9622 respectively, on the ACL-BioNLP workshop MediQA Question Answering shared-task.

==> sections/Contribution.tex <==
\section{Contribution}

\begin{table}[h!]
\centering
\begin{adjustbox}{width=0.49\textwidth}
\begin{tabular}{|l|l|}
\hline
\textbf{Team Members} & \textbf{Task}                   \\ \hline
Karan and Shefali       & Natural Language Inference      \\ \hline
Prashant and Sheetal    & Recognizing Question Entailment \\ \hline
Hemant                & Question Re-ranking and Filtering    \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}
